Seeing the World through Your Eyes

The reflective nature of the human eye is an underappreciated source of information about what the world around us looks like. By imaging the eyes of a moving person, we can collect multiple views of a scene outside the camera's direct line of sight through the reflections in the eyes. In this paper, we reconstruct a 3D scene beyond the camera's line of sight using portrait images containing eye reflections. This task is challenging due to 1) the difficulty of accurately estimating eye poses and 2) the entangled appearance of the eye iris and the scene reflections. Our method jointly refines the cornea poses, the radiance field depicting the scene, and the observer's eye iris texture. We further propose a simple regularization prior on the iris texture pattern to improve reconstruction quality. Through various experiments on synthetic and real-world captures featuring people with varied eye colors, we demonstrate the feasibility of our approach to recover 3D scenes using eye reflections.

==> figures/pose_optimization.tex <==
\begin{figure}
\begin{center}
\centering

% \includegraphics[width=\linewidth]{images/Why_figure.pdf}
% \mpage{0.49}{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/andrew_no_opt_cropped.png}}\hfill
% \mpage{0.49}{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/andrew_front_cropped.png}}\hfill
\mpage{0.49}{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/lit_plushies_no_pose_zoomed.png}}\hfill
\mpage{0.49}{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/lit_plushies_opt.png}}\hfill
    \mpage{0.49}{\sffamily No cornea pose optimization} \hfill 
    \mpage{0.48}{\sffamily With cornea pose optimization}
\captionof{figure}{
\textbf{Effect of cornea pose optimization.} 
On real data, the reconstruction results in poor quality without jointly optimizing for the cornea poses throughout training due to the small cornea size. 
Here we show that our cornea pose optimization is critical to performance.
}

\label{fig:pose_optim}
\end{center}
\end{figure}


==> figures/texture_decomposition.tex <==
\begin{figure}
\begin{center}
\centering

% \includegraphics[width=\linewidth]{images/Why_figure.pdf}
\mpage{0.49}{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/no_texture_andrew_light.png}}\hfill
\mpage{0.49}{\includegraphics[width=\linewidth, trim=0 0 0 0, clip]{images/texture_andrew_light.png}}\hfill
    \mpage{0.47}{\sffamily No texture decomposition} \hfill 
    \mpage{0.47}{\sffamily With texture decomposition}
\captionof{figure}{
\textbf{Effects of texture decomposition.} Learning an explicit estimate of the iris texture is essential to reducing floaters in the rendering views and learning a better scene geometry.}

\label{fig:texture_decomposition}
\end{center}
\end{figure}

